Persona-based Assessment of Software Engineering Student Research Projects: An Experience Report

Students enrolled in software engineering degrees are generally required to undertake a research project in their final year through which they demonstrate the ability to conduct research, communicate outcomes, and build in-depth expertise in an area. Assessment in these projects typically involves evaluating the product of their research via a thesis or a similar artifact. However, this misses a range of other factors that go into producing successful software engineers and researchers. Incorporating aspects such as process, attitudes, project complexity, and supervision support into the assessment can provide a more holistic evaluation of the performance likely to better align with the intended learning outcomes. In this paper, we present on our experience of adopting an innovative assessment approach to enhance learning outcomes and research performance in our software engineering research projects. Our approach adopted a task-oriented approach to portfolio assessment that incorporates student personas, frequent formative feedback, delayed summative grading, and standards-aligned outcomes-based assessment. We report upon our continuous improvement journey in adapting tasks and criteria to address the challenges of assessing student research projects. Our lessons learnt demonstrate the value of personas to guide the development of holistic rubrics, giving meaning to grades and focusing staff and student attention on attitudes and skills rather than a product only.

==> Files/ICSE_instructions.tex <==


Experience Report (max 10 pages, plus up to 2 pages for references) An experience report provides anecdotal evidence by describing an experience related to software engineering education and training (typically a course, a teaching or training technique or strategy, or an assessment method) and interprets the experience in terms of actionable advice and lessons learned, but does not need to evaluate it or use rigorous research methods to support its claims. Negative and mixed findings are acceptable provided they can support advice or lessons learned.

Evaluation Criteria
Submissions will be evaluated based on their category:

Experience Reports will be evaluated against these criteria: Relevance, Significance, Actionability, Lessons, Presentation

The evaluation criteria for SEET 2023 papers are defined as follows:

● Relevance: The extent to which the paper is relevant to SEET.

● Significance: The extent to which the paper is well-motivated and its contributions are original and important, with respect to the existing literature on software engineering education and training.

● Actionability: The extent to which the paper provides actionable advice with clear take-away messages.

● Lessons: The extent to which the paper meaningfully discusses lessons learned in terms of what went right, what went wrong, and what could be improved if the experience is repeated.

● Presentation: The extent to which the paper’s organization and quality of writing is up to the standard: the paper is well-structured, employs clear and correct scholarly language, avoids ambiguity, includes clearly readable figures and tables, and is appropriately formatted.

---------------------------------------------------------------------
Research Papers will be evaluated against these criteria: Relevance, Significance, Soundness, Verifiability, Presentation

● Soundness: The extent to which the paper’s contributions are supported by rigorous application of appropriate research methods and whether the paper discusses meaningfully the research methods’ limitations and threats to the validity of the findings.

● Verifiability: The extent to which the paper includes sufficient information to support independent verification or replication of the paper’s claimed contributions. This includes public availability of research data or an explicit statement why such data cannot be made publicly available.

● Maturity: The extent to which the tool or technology is mature enough to be presented.

● Availability: Whether the tool or technology is available online, open-sourced, or on a trial basis and the extent to which it can be evaluated by potential users.

==> Files/backup_text.tex <==
\subsection{Empathize Stage}

The first step in the design thinking approach is empathise and involves understanding the problem and users’ needs, experiences, behaviors and goals. Conversations among academics and curriculum design experts identified two main issues with the research units:

1. Assessment focus. The existing assessment model was analysed and the excessive focus on the end-product, i.e., ``research thesis'' was highlighted, in contrast to the little focus on improving students' research skills. Looking back at the unit learning outcomes it is clear that the goal of these units is to provide students with a learning environment that allows them to develop the skills required for independent research. Existing literature on assessment grids and researchers' personas~\cite{Willison:12, Guetterman:17}, research process in computer science or IT~\cite{Ramesh:04, Wohlin:12}, together with our own and our colleagues experiences were used to identify the key skills and processes required for independent research. This process resulted in the identification of seven important aspects: literature review, technical and academic writing, research design, project management, artefact development, research evaluation, and research dissemination. 

2. Varied level of guidance required by our students. Some students are able to grasp the higher level requirements of research projects and work independently, while other students expect clear instructions for each step of the process, not being able to develop their own plan or see the research project as a whole. We aligned these observations with the concept of agency, defined through a social cognitive lens as the ability to exert control over, and direct, ones own learning \cite{biesta2007agency,etelapelto2013agency}. An important aspect of agency as viewed through a social cognitive perspective is its developmental nature \cite{bandura2006adolescent}. Kegan’s constructive developmental theory analyses developmental changes through adulthood in terms of evolvement and exercise of human agency \cite{kegan1994}. According to Kegan's stages of adult development, students in higher education present: instrumental, socialised and self-authoring minds (See Table \ref{table:Kegan}). In our assessment design we will use Kegan's stages to understand how to better support and challenge our students holistically \cite{kegan1994,magolda2004making}.

\begin{table*}[htbp]
\centering
\caption{Robert Kegan's developmental stages}
\label{table:Kegan}
\begin{center}
\scriptsize
\begin{tabular}{ |p{3cm}|p{13cm}| }
 \hline
 \textbf{Developmental stage} & \textbf{Characteristics}
 \\
 \hline
 Instrumental mind  
 & Students commonly make decisions based on the benefits or consequences that may result from these, thus needing authority figures or rules to direct them.  
 \\
  \hline
Socialised mind  
 & Students are ``good citizens'', taking others into account and considering long term consequences. They understand others' points of view, even if different from their own.  
 \\
\hline
Self-authoring mind  
 & Students can evaluate arguments (their own and others’) using evidence, take contextual factors into account, acknowledge multiple ways of framing arguments, and reevaluate the basis of a decision as evidence changes.  
\\
  \hline
 \end{tabular}
 \end{center}
 \end{table*}


%%%%%%%%
\sectopic{Design Thinking: Define Stage}

In the define stage of design thinking the information collected needs to be synthesised. In this case we have identified research skills and processes that our students need to develop, and we have our personas, representing the agency profiles of students present in our cohorts. These two aspects will come together in a rubric. The first step for this synthesis is to create research-specific personas, these research-specific personas represent the agency through attitudes and behaviours, that our different students will demonstrate in the context of research according to their agentic characteristics. The resulting research personas are presented in Figure \ref{fig:personas}. The identified research personas are aligned to a grade and presented at the top of the rubric. They are used to guide the creation of the descriptors within the rubric and communicate high-level attributes of each persona to students. The rows of the rubric capture the domain-specific learning outcomes, or assessment criteria of the rubric. These criteria are derived from the seven aspects required for research, which are aligned with the research unit's learning outcomes, and capture the dimensions through which students are going to be assessed. 

Once the grade-based personas and criteria are identified, and captured in the rubric, the next step is to provide descriptors for the expectations of each criteria, at each grade level. The personas characteristics are used to determine the knowledge, skills and dispositions that students need to demonstrate at each level of achievement for that particular criteria. With the integration of the persona model for rubric development, the qualitative differences across achievement levels are holistic, merging the intrapersonal, interpersonal and cognitive dimensions. This rubric clearly states that to achieve a higher grade students need to be more independent in their research and learning (See Figure \ref{fig:personas}). 
Figure~\ref{fig:Rubric} shows an excerpt from the assessment rubric for the `Literature Review' criterion at different grade levels.

\begin{figure*}
    \centering
    %\vspace*{30em}
    %\hspace*{-70em}
    %\begin{tikzpicture}[scale=1]
        \includegraphics[width=2\columnwidth]{Figures/ResearchPersonas.png}
    %\end{tikzpicture}
\caption{Research Personas.} 
\label{fig:personas} 
\end{figure*}


In this case we identified research skills and processes that our students need to develop, and we have our personas, representing the agency profiles of students present in our cohorts. These two aspects will come together in a rubric. The first step for this synthesis is to create research-specific personas, these research-specific personas represent the agency through attitudes and behaviours, that our different students will demonstrate in the context of research according to their agentic characteristics. The resulting research personas are presented in Figure \ref{fig:personas}. The identified research personas are aligned to a grade and presented at the top of the rubric. They are used to guide the creation of the descriptors within the rubric and communicate high-level attributes of each persona to students. The rows of the rubric capture the domain-specific learning outcomes, or assessment criteria of the rubric. These criteria are derived from the seven aspects required for research, which are aligned with the research unit's learning outcomes, and capture the dimensions through which students are going to be assessed. 

Once the grade-based personas and criteria are identified, and captured in the rubric, the next step is to provide descriptors for the expectations of each criteria, at each grade level. The personas characteristics are used to determine the knowledge, skills and dispositions that students need to demonstrate at each level of achievement for that particular criteria. With the integration of the persona model for rubric development, the qualitative differences across achievement levels are holistic, merging the intrapersonal, interpersonal and cognitive dimensions. This rubric clearly states that to achieve a higher grade students need to be more independent in their research and learning (See Figure \ref{fig:personas}). 
Figure~\ref{fig:Rubric} shows an excerpt from the assessment rubric for the `Literature Review' criterion at different grade levels.

\newpage

%We aligned these observations with the concept of agency, defined through a social cognitive lens as the ability to exert control over, and direct, ones own learning \cite{biesta2007agency,etelapelto2013agency}. An important aspect of agency as viewed through a social cognitive perspective is its developmental nature \cite{bandura2006adolescent}. Kegan’s constructive developmental theory analyses developmental changes through adulthood in terms of evolvement and exercise of human agency \cite{kegan1994}. According to Kegan's stages of adult development, students in higher education present: instrumental, socialised and self-authoring minds (See Table \ref{table:Kegan}). In our assessment design we will use Kegan's stages to understand how to better support and challenge our students holistically~\cite{kegan1994,magolda2004making}.

%Looking back at the unit learning outcomes it is clear that the goal of these units is to provide students with a learning environment that allows them to develop the skills required for independent research. Existing literature on assessment grids and researchers' personas~\cite{Willison:12, Guetterman:17}, research process in computer science or IT~\cite{Ramesh:04, Wohlin:12}, together with our own and our colleagues experiences were used to identify the key skills and processes required for independent research. This process resulted in the identification of seven important aspects: literature review, technical and academic writing, research design, project management, artefact development, research evaluation, and research dissemination. 

%The first step in the design thinking approach is empathise and involves understanding the problem and users’ needs, experiences, behaviors and goals. Conversations among academics and curriculum design experts identified two main issues with the research units:






% \sectopic{Rubric and persona model}



\sectopic{Motivation for assessment redesign}

The assessment model in place in these units before 2019 did not seem to be working for learning nor grading. 

Learning- problems getting students to finish projects? something around that?

Grading- Results were not accurate, with the grade distribution not reflecting our observations of the level of our students. Although  x \% of students obtained high grades (80 \% or higher), most students did not appear to meet the level of achievement represented by that grade. This inaccuracy could have been due to contract cheating or other integrity issues \cite{}, exacerbated by the fact that the assessment for this unit focused on summative assessment of the research thesis, without any intermediate checkpoints and submissions \cite{}. In addition, this assessment model was not equitable. Supervisors appeared to be biased towards their students, and might have a vested interest in higher grades for their students as these can translate to PhD scholarships -- a common issue in the fairness of assessment~\cite{Green:10}. Inaccuracy, potential academic integrity, and potential bias resulted in students being considered research-ready when they were not, including students who entered the PhD program. If not addressed, the overall reputation of the software engineering research graduates would be impacted by this. To alleviate these issues, we worked on designing a new assessment model for these units using a design thinking approach \cite{}. 





% To support assessment design in professional units, a course level set of personas and criteria was created that helps align assessment qualities across units. These persona characteristics align with the course learning outcomes and drive the creation of persona-based developmental rubrics that provide students and staff with coherent representations of qualities associated with each grade in a way that is meaningful, approachable and easy to understand. This resulted in a consistent distinction between grades across units in a course. It also changed the way educators think about their role, the role of assessment and what consists evidence of learning.


% The \textit{persona} model presents capabilities as being linked to a specific developmental stage. This presents a holistic view of capabilities, allowing an easy alignment of intangible and tangible components of the capabilities. Intangible components of capabilities include behaviours and dispositions, while more tangible components include knowledge and skills, which are more easily determined through performance and outputs. The visibility that this model provides to the intangible components of the capabilities allows for an easier incorporation of these into learning and assessment design. 

% The change in mindset comes from shifting the view of capabilities from a sum of components, to viewing them as a coherent whole. This highlights the importance of behaviours and dispositions, further supporting the importance of intentionally addressing these and not only students' cognitive development. Additionally, by providing coherent representations of qualities associated with each grade, grades are given meaning both in terms of students' demonstrated capabilities, as well as in terms of the discipline's aspirational capabilities. In doing so, the role of higher education expands to a more holistic endeavour as opposed to focusing on knowledge transmission.



\sectopic{Design Thinking: Define Stage}

In the define stage of design thinking the information collected needs to be synthesised. In this case we have identified research skills and processes that our students need to develop, and we have our personas, representing the agency profiles of students present in our cohorts. These two aspects will come together in a rubric. The first step for this synthesis is to create research-specific personas, these research-specific personas represent the agency through attitudes and behaviours, that our different students will demonstrate in the context of research according to their agentic characteristics. The resulting research personas are presented in Figure \ref{fig:personas}. The identified research personas are aligned to a grade and presented at the top of the rubric. They are used to guide the creation of the descriptors within the rubric and communicate high-level attributes of each persona to students. The rows of the rubric capture the domain-specific learning outcomes, or assessment criteria of the rubric. These criteria are derived from the seven aspects required for research, which are aligned with the research unit's learning outcomes, and capture the dimensions through which students are going to be assessed. 

Once the grade-based personas and criteria are identified, and captured in the rubric, the next step is to provide descriptors for the expectations of each criteria, at each grade level. The personas characteristics are used to determine the knowledge, skills and dispositions that students need to demonstrate at each level of achievement for that particular criteria. With the integration of the persona model for rubric development, the qualitative differences across achievement levels are holistic, merging the intrapersonal, interpersonal and cognitive dimensions. This rubric clearly states that to achieve a higher grade students need to be more independent in their research and learning (See Figure \ref{fig:personas}). 
Figure~\ref{fig:Rubric} shows an excerpt from the assessment rubric for the `Literature Review' criterion at different grade levels.

\begin{figure*}
    \centering
    %\vspace*{30em}
    %\hspace*{-70em}
    %\begin{tikzpicture}[scale=1]
        \includegraphics[width=2\columnwidth]{Figures/ResearchPersonas.png}
    %\end{tikzpicture}
\caption{Research Personas.} 
\label{fig:personas} 
\end{figure*}

\sectopic{Design Thinking: Ideate Stage}

At this stage, we have defined our students, learning outcomes, and the achievement levels expected. The brainstorming is now focused on developing our solution, in this case, the assessment tasks that would support the students in achieving the unit learning outcomes and in demonstrating their achievements. The main issue in the previous assessment design was that the students were being assessed only on the end-product, i.e., ``research thesis'', with little focus on guiding them through the research process or on assessing their research skills. The Task-Oriented Portfolio Assessment Model  (TOPAM) \cite{cain2020using} is a process-oriented assessment model. It addresses a few of our issues, such as the development of skills through its iterative feedback loops, development and assessment of every criterion through outcome-based assessment, and supporting the needs of our varied cohort through differentiated tasks. It was decided that this model would be used and we created tasks to guide student learning at the different levels of achievement.



In this step, we have defined our students, learning outcomes, and the achievement levels expected. The brainstorming is now focused on developing our solution, in this case, the assessment tasks that would support the students in achieving the unit learning outcomes and in demonstrating their achievements. The main issue in the previous assessment design was that the students were being assessed only on the end-product, i.e., ``research thesis'', with little focus on guiding them through the research process or on assessing their research skills. The Task-Oriented Portfolio Assessment Model  (TOPAM) \cite{cain2020using} is a process-oriented assessment model. It addresses a few of our issues, such as the development of skills through its iterative feedback loops, development and assessment of every criterion through outcome-based assessment, and supporting the needs of our varied cohort through differentiated tasks. It was decided that this model would be used and we created tasks to guide student learning at the different levels of achievement.


\subsection{Research Unit (\unitcode) Context}~\label{subsec:UnitContext}

To allow them to develop basic research skills, prior to this unit, Software Engineering students at our university undertake a unit that covers research training and project management. This unit aims to help them develop the skills necessary to undertake a Software Engineering research project. The focus is on allowing students to explore an area of interest by defining their own project scope and direction.  They develop literature search skills, academic writing skills, data analysis skills, presentation, and experiment design skills

Whilst developing these skills, students are encouraged to explore the area of Software Engineering that is of most interest to them and ultimately develop a research plan and proposal. We have found that this hybrid approach of learning about research whilst exploring an area and developing a proposal allows lots of flexibility for Software Engineering students. 

==> Files/relevantPapers.tex <==
%%Other Relevant Papers
https://dl.acm.org/doi/fullHtml/10.1145/3416465.3416469

